Coding and tiling of Julia sets for subhyperbolic rational maps

Let $f:\hat{C}\to\hat{C}$ be a subhyperbolic rational map of degree $d$. We construct a set of coding maps $Cod(f)=\{\pi_r:\Sigma\to J\}_r$ of the Julia set $J$ by geometric coding trees, where the parameter $r$ ranges over mappings from a certain tree to the Riemann sphere. Using the universal covering space $\phi:\tilde S\to S$ for the corresponding orbifold, we lift the inverse of $f$ to an iterated function system $I=(g_i)_{i=1,2,...,d}$. For the purpose of studying the structure of $Cod(f)$, we generalize Kenyon and Lagarias-Wang's results : If the attractor $K$ of $I$ has positive measure, then $K$ tiles $\phi^{-1}(J)$, and the multiplicity of $\pi_r$ is well-defined. Moreover, we see that the equivalence relation induced by $\pi_r$ is described by a finite directed graph, and give a necessary and sufficient condition for two coding maps $\pi_r$ and $\pi_{r'}$ to be equal.

==> cod <==
\\
Title: Coding and tiling of Julia sets for subhyperbolic rational maps
Authors: Atsushi Kameyama
Comments: 27 pages, 5 figures
Report-no:
Subj-class: Dynamical systems
Journal-ref: 
MSC-class: 37F20 (Primary) 28A80 (Secondary)
\\
 Let $f:\hat{\mathbb C}\to\hat{\mathbb C}$ be a subhyperbolic rational map of degree $d$.
We construct a set of coding maps $\mathrm{Cod}(f)=\{\pi_r:\Sigma\to J\}_r$ of 
the Julia set $J$ by geometric coding trees, where the parameter $r$ ranges over mappings from a certain tree to the Riemann sphere.
Using the universal covering space $\phi:\tilde S\to S$ for the corresponding orbifold, we lift the inverse of $f$  to an iterated function system $\mathcal I=(g_i)_{i=1,2,\dots,d}$. 
For the purpose of studying the structure of $\mathrm{Cod}(f)$, we generalize Kenyon and Lagarias-Wang's results : If the attractor $K$ of $\mathcal I$ has positive measure, then $K$ tiles $\phi^{-1}(J)$, and the multiplicity of $\pi_r$ is well-defined.
Moreover, we see that the equivalence relation induced by $\pi_r$ is described  by a finite directed graph, and give a necessary and sufficient condition for two coding maps $\pi_r$ and $\pi_{r'}$ to be equal.
\\

